RTFF: Random-to-Target Fabric Flattening Policy using Dual-Arm Manipulator

Robotic fabric manipulation remains challenging due to fabric deformability and occlusions from wrinkles and the manipulator. This paper defines Random-to-Target Fabric Flattening (RTFF) as the task of bringing a randomly wrinkled fabric to an arbitrary user-specified wrinkle-free target pose. RTFF requires simultaneous flattening and pose alignment, where the two objectives are inherently coupled since flattening the fabric displaces its pose, while realigning it tends to introduce wrinkles. To solve this task, this paper anchors both the current and target fabric states to the same template mesh, enabling direct vertex-level wrinkle and pose assessment without registration. Building on this representation, a hybrid Imitation Learning--Visual Servoing (IL--VS) RTFF policy is proposed. A novel Mesh Action Chunking Transformer (MACT) leverages structured mesh observations to achieve goal-conditioned coarse alignment from a compact demonstration set, after which VS ensures precise convergence to the target. The policy is validated on a real dual-arm teleoperation system, demonstrating precise alignment to unseen target poses, fabric types, and scales. Code and videos: https://kaitang98.github.io/RTFF_Policy/

==> utils/utils.tex <==
\begin{table}[h]
    \centering
    \caption{Mesh prediction under increasing occlusion.}
    \label{tab:sim_occlusion}
    \renewcommand{\arraystretch}{0.85}
    \setlength{\tabcolsep}{4pt}
    \resizebox{0.5\columnwidth}{!}{%
    \begin{tabular}{c c c c}
    \toprule
    \textbf{Occlusion} & \textbf{MVE [m]} & \textbf{MKE [m]} & \textbf{OCD [m]} \\
    \midrule
      0\%  & 0.0042 & 0.0048 & 0.0082 \\
      5\%  & 0.0050 & 0.0059 & 0.0093 \\
     10\%  & 0.0056 & 0.0067 & 0.0102 \\
     20\%  & 0.0070 & 0.0084 & 0.0120 \\
     30\%  & 0.0088 & 0.0107 & 0.0133 \\
     40\%  & 0.0111 & 0.0139 & 0.0146 \\
    \midrule
     50\%  & 0.0153 & 0.0197 & 0.0183 \\
     60\%  & 0.0245 & 0.0297 & 0.0220 \\
     70\%  & 0.0313 & 0.0431 & 0.0274 \\
     80\%  & 0.0431 & 0.0604 & 0.0327 \\
     90\%  & 0.0558 & 0.0889 & 0.0450 \\
    100\%  & 0.0684 & 0.1057 & 0.0583 \\
    \bottomrule
    \end{tabular}}
\end{table}



\begin{table}[h]
\centering
\caption{Real-world prediction under increasing occlusion.}
\label{tab:real_occlusion}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{0.9}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{c c c c}
\toprule
\textbf{Occlusion} & \textbf{CD before [m]} & \textbf{CD after [m]} & \textbf{Improv. [\%]} \\
& \textbf{(mean \(\pm\) std)} & \textbf{(mean \(\pm\) std)} & \\
\midrule
  0\% & \(0.0131 \pm 0.0008\) & \(0.0095 \pm 0.0001\) & 28.0 \\
 10\% & \(0.0146 \pm 0.0013\) & \(0.0105 \pm 0.0005\) & 28.4 \\
 20\% & \(0.0152 \pm 0.0017\) & \(0.0115 \pm 0.0011\) & 24.6 \\
 30\% & \(0.0180 \pm 0.0031\) & \(0.0124 \pm 0.0017\) & 31.2 \\
 40\% & \(0.0177 \pm 0.0041\) & \(0.0135 \pm 0.0028\) & 23.5 \\
 50\% & \(0.0266 \pm 0.0077\) & \(0.0210 \pm 0.0065\) & 21.0 \\
\bottomrule
\end{tabular}%
}
\end{table}


% \begin{table}[h]
% \centering
% \caption{Real-world Chamfer distance (mean \(\pm\) std, in metres) before/after refinement under increasing occlusion.}
% \label{tab:real_occlusion}
% \setlength{\tabcolsep}{3.5pt}
% \renewcommand{\arraystretch}{0.9}
% \resizebox{0.7\columnwidth}{!}{%
% \begin{tabular}{c c c c}
% \toprule
% \textbf{Occlusion} & \textbf{CD (before)} & \textbf{CD (after)} & \textbf{Improvement} \\
% \midrule
%   0\% & \(0.0131 \pm 0.0008\) & \(0.0095 \pm 0.0001\) & 28.0\% \\
%  10\% & \(0.0146 \pm 0.0013\) & \(0.0105 \pm 0.0005\) & 28.4\% \\
%  20\% & \(0.0152 \pm 0.0017\) & \(0.0115 \pm 0.0011\) & 24.6\% \\
%  30\% & \(0.0180 \pm 0.0031\) & \(0.0124 \pm 0.0017\) & 31.2\% \\
%  40\% & \(0.0177 \pm 0.0041\) & \(0.0135 \pm 0.0028\) & 23.5\% \\
%  50\% & \(0.0266 \pm 0.0077\) & \(0.0210 \pm 0.0065\) & 21.0\% \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table}[h]
% \centering
% \caption{Real-world Chamfer distance (m) before/after refinement under increasing occlusion.}
% \label{tab:real_occlusion}
% \footnotesize
% \setlength{\tabcolsep}{3.5pt}
% \renewcommand{\arraystretch}{0.9}
% \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{c c c c}
% \toprule
% \textbf{Occlusion} &
% \textbf{CD before (mean \(\pm\) std) [m]} &
% \textbf{CD after (mean \(\pm\) std) [m]} &
% \textbf{Improv. [\%]} \\
% \midrule
%   0\% & \(0.0131 \pm 0.0008\) & \(0.0095 \pm 0.0001\) & 28.0 \\
%  10\% & \(0.0146 \pm 0.0013\) & \(0.0105 \pm 0.0005\) & 28.4 \\
%  20\% & \(0.0152 \pm 0.0017\) & \(0.0115 \pm 0.0011\) & 24.6 \\
%  30\% & \(0.0180 \pm 0.0031\) & \(0.0124 \pm 0.0017\) & 31.2 \\
%  40\% & \(0.0177 \pm 0.0041\) & \(0.0135 \pm 0.0028\) & 23.5 \\
%  50\% & \(0.0266 \pm 0.0077\) & \(0.0210 \pm 0.0065\) & 21.0 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


From Intro 
% ---- 2. Template mesh: DEFINES the task, not merely enables it ------
%        [K2, §3.4 – mesh central to task definition & state estimation]
%        [RC 1.2 – prominent early; RC 1.3 – application not invention]
The major limitation of existing methods is the lack of shared geometric reference between the observed fabric and the target.
This paper proposes to define both the current fabric state and the target configuration as instances of the same \textit{template mesh}, a canonical mesh derived from the fabric's CAD model that deforms to match any observed state while preserving vertex identity.
Prior work~\cite{wang2024trtm} used template meshes only for state tracking; the key contribution here is to also anchor the target pose to the same mesh,
so that local wrinkle presence and pose offset can be read directly from
vertex-level differences between the current and target mesh instances~(R1, R3),
and a mesh-derived flatness criterion provides a continuous signal for automatically
switching between wrinkle removal and fine alignment within one policy~(R2).

Building on this formulation, this paper proposes a two-stage RTFF policy: an
\ac{IL} stage, implemented as \textit{\acf{MACT}}, that learns from a small
demonstration set to perform coarse wrinkle removal guided by the mesh state;
followed by a \ac{VS} stage that activates once the mesh signals sufficient
flatness and drives the fabric to precise alignment with the target.
\ac{MACT} adapts the ACT architecture~\cite{zhao2023learning} to take mesh
state and alignment error as inputs in place of raw images.
% 
The contributions of this paper are:
\begin{itemize}
    \item A template-mesh formulation of RTFF that anchors both the current and
    target states to the same canonical mesh, enabling direct local wrinkle and
    pose assessment without registration, and a mesh-driven hybrid \ac{IL}--\ac{VS}
    policy with automatic switching.
    \item \ac{MACT}, a mesh-conditioned action chunking transformer that achieves
    goal-conditioned RTFF from a compact demonstration set; ablation studies confirm
    mesh input is essential to task success.
    \item Physical validation on a real dual-arm system across varying wrinkle
    complexities, demonstrating zero-shot generalisation to unseen target
    configurations and across different fabrics.
\end{itemize}

\section{Other nonsense from introduction}

% Why IL can help (only the main reason)
Recently, \textit{\ac{IL}} has become popular for fabric manipulation such as flattening~\cite{Seita2020} and folding~\cite{black2024pi_0}. By learning the observation-action mapping directly from expert demonstrations, IL eliminates the need for explicit models of fabric deformability and dynamics. Thus, IL demonstrates promising potential in RTFF, for example, transforming a wrinkled fabric to a wrinkle-free state, enabling coarse alignment, and providing demonstration-informed grasping points to VS.
%
However, IL faces two key challenges in RTFF: 
%
i) most existing IL approaches ~\cite{zhao2023learning, zhao2024aloha, Ze2024DP3, black2024pi_0} generate a sequence of actions (referred to as an \textit{action chunk}), by directly conditioned on RGB or RGB-D images, which limits the ability of IL policies to specify various targets, identify robust wrinkle features from fabric images and to track alignment errors between the fabric current and target state;
%
ii) achieving both high-precision manipulation and generalization across diverse wrinkled fabric and target states typically requires large, costly datasets of expert demonstrations~\cite{zhao2024aloha}.

% combine IL and VS
Consequently, a natural direction is a hybrid IL–VS policy that leverages the strengths of both paradigms for RTFF: IL is first used to flatten the initially wrinkled fabric and obtain \textit{coarse alignment}, followed by VS to achieve \textit{fine alignment}. The primary challenge in realizing this integration is accurate and efficient fabric \textit{state estimation}, since both paradigms require a consistent geometric representation of the fabric for precise RTFF problem formulation and fabric manipulation and alignment, which is the key bridge to a unified RTFF policy.
% Challenges state estimation
However, fabric state estimation is challenging due to fabric’s effectively infinite \ac{DoF}. Additionally, \textit{self-occlusions} from wrinkles and folds and \textit{external-occlusions} from the manipulator’s \ac{EE} and arm during RTFF, obscure fabric perception and thereby limit state estimation.
